Improving the Improver: Semantic PID Control for Medical Agent Self-Improvement

High-stakes vertical medical tasks, such as postoperative pathological staging and long-term survival prediction, demand multi-step clinical reasoning over heterogeneous evidence under weak supervision and high outcome uncertainty. While we first orchestrate CliAgent, a domain-tailored clinical agent workflow that systematically grounds predictions in multi-modal patient evidence, manually designed medical agents remain constrained by static, brittle rules. Moreover, existing recursive self-improvement (RSI) methods suffer from feedback ambiguity and severe development-set overfitting when evolving agents in high-noise medical domains. Focusing on improving the improver, we propose Semantic PID-RSI, an evidence-guided control-theoretic framework for medical agent self-improvement. Inspired by PID control, our improver evaluates candidate modification batches via three diagnostic roles: P isolates current clinical failure modes, I synthesizes longitudinal evidence from past trials, and D estimates response dynamics and regression risks (D-pre/D-post). Selected plans are compiled into behavior contracts for staged probing and independent adoption judging. Instantiated and validated on challenging oncology tasks (pT/pN staging and survival prognosis), evolving CliAgent with Semantic PID-RSI on a 3B-activated open-weight model achieves substantial gains (up to +6.27 C-index points), outperforming overfitting-prone RSI baselines and approaching the performance of frontier proprietary models (e.g., GPT-6 series) equipped with CliAgent.

==> pidinner/preamble.tex <==
\ifdefined\PIDRSIImportLoaded
\else
\def\PIDRSIImportLoaded{1}
\makeatletter
\@ifpackageloaded{graphicx}{}{\RequirePackage{graphicx}}
\@ifpackageloaded{amsmath}{}{\RequirePackage{amsmath}}
\@ifpackageloaded{amssymb}{}{\RequirePackage{amssymb}}
\@ifpackageloaded{mathtools}{}{\RequirePackage{mathtools}}
\@ifpackageloaded{booktabs}{}{\RequirePackage{booktabs}}
\@ifpackageloaded{multirow}{}{\RequirePackage{multirow}}
\@ifpackageloaded{enumitem}{}{\RequirePackage{enumitem}}
\@ifpackageloaded{xcolor}{}{\RequirePackage{xcolor}}
\makeatother

\newcommand{\PIDRSITodo}[1]{\textcolor{red}{\textbf{[TODO: #1]}}}
\newcommand{\PIDRSIMethod}{Semantic PID-RSI}
\newcommand{\PIDRSITaskProgram}{H}
\newcommand{\PIDRSIImprover}{S}
\newcommand{\PIDRSIProtocol}{\Pi}
\newcommand{\PIDRSIEvidence}{\mathcal{E}}
\newcommand{\PIDRSIMetaEvidence}{\mathcal{M}}
\newcommand{\PIDRSIOffspring}{\mathcal{O}}
\fi

